An ADM 3+1 formulation for Smooth Lattice General Relativity

A new hybrid scheme for numerical relativity will be presented. The scheme will employ a 3-dimensional spacelike lattice to record the 3-metric while using the standard 3+1 ADM equations to evolve the lattice. Each time step will involve three basic steps. First, the coordinate quantities such as the Riemann and extrinsic curvatures are extracted from the lattice. Second, the 3+1 ADM equations are used to evolve the coordinate data, and finally, the coordinate data is used to update the scalar data on the lattice (such as the leg lengths). The scheme will be presented only for the case of vacuum spacetime though there is no reason why it could not be extended to non-vacuum spacetimes. The scheme allows any choice for the lapse function and shift vectors. An example for the Kasner $T^3$ cosmology will be presented and it will be shown that the method has, for this simple example, zero discretisation error.

==> gr-qc.tex <==
%
\catcode`@=11%
%
\def\defineten{%
   \font\tentext=cmr10 scaled 1000%
   \font\tenscript=cmr7 scaled 1000%
   \font\tenscriptscript=cmr5 scaled 1000%
   \font\tenmathtext=cmmi10 scaled 1000%
   \font\tenmathscript=cmmi7 scaled 1000%
   \font\tenmathscriptscript=cmmi5 scaled 1000%
   \font\tensymboltext=cmsy10 scaled 1000%
   \font\tensymbolscript=cmsy7 scaled 1000%
   \font\tensymbolscriptscript=cmsy5 scaled 1000%
   \font\tenmathex=cmex10 scaled 1000%
   \font\tenboldtext=cmbx10 scaled 1000%
   \font\tenboldscript=cmbx7 scaled 1000%
   \font\tenboldscriptscript=cmbx5 scaled 1000%
   \font\tenslant=cmsl10 scaled 1000%
   \font\tenitalic=cmti10 scaled 1000%
   \font\tentypewriter=cmtt10 scaled 1000%
% Set skew and hyphenation characters
   \skewchar\tenmathtext='177%
   \skewchar\tenmathscript='177%
   \skewchar\tenmathscriptscript='177%
   \skewchar\tensymboltext='60%
   \skewchar\tensymbolscript='60%
   \skewchar\tensymbolscriptscript='60%
   \hyphenchar\tentypewriter=-1%
}% \global\let\defineten=\relax}%
%
\def\tenpoint{%
   \defineten%
   \textfont0=\tentext \scriptfont0=\tenscript%
      \scriptscriptfont0=\tenscriptscript%
   \def\rm{\fam0 \tentext}%%
   \textfont1=\tenmathtext \scriptfont1=\tenmathscript%
      \scriptscriptfont1=\tenmathscriptscript%
   \textfont2=\tensymboltext \scriptfont2=\tensymbolscript%
      \scriptscriptfont2=\tensymbolscriptscript%
   \textfont3=\tenmathex \scriptfont3=\tenmathex%
      \scriptscriptfont3=\tenmathex%
   \textfont\bffam=\tenboldtext \scriptfont\bffam=\tenboldscript%
      \scriptscriptfont\bffam=\tenboldscriptscript%
   \def\bf{\fam\bffam\tenboldtext}%
   \textfont\itfam=\tenitalic \def\it{\fam\itfam\tenitalic}%
   \textfont\slfam=\tenslant \def\sl{\fam\slfam\tenslant}%
   \textfont\ttfam=\tentypewriter \def\tt{\fam\ttfam\tentypewriter}%
%Set up \mit, \oldstyle, \cal
   \def\mit{\fam1 }\def\oldstyle{\fam1 \tenmathtextfont}%
   \def\cal{\fam2 }%
%Set up big etc.
\def\big##1{{\hbox{$\left##1\vbox to 8.5pt{}\right.\n@space$}}}%
\def\Big##1{{\hbox{$\left##1\vbox to 11.5pt{}\right.\n@space$}}}%
\def\bigg##1{{\hbox{$\left##1\vbox to 14.5pt{}\right.\n@space$}}}%
\def\Bigg##1{{\hbox{$\left##1\vbox to 17.5pt{}\right.\n@space$}}}%
%
%Now define a strut box for tenpt
   \setbox\strutbox=\hbox{\vrule height 8.5pt depth 3.5pt width0pt}%
   \normalbaselineskip=12pt%
   \normalbaselines\rm%
}
%
\catcode`@=12% Back to normal
%
% Double space macro for 12 point font.
%
    \gdef\twelvepointdbl{%
         \twelvepoint%
         \abovedisplayskip 18pt plus 4pt minus 6pt%
         \belowdisplayskip 18pt plus 4pt minus 6pt%
         \abovedisplayshortskip  0pt plus 4pt%
         \belowdisplayshortskip 10pt plus 4pt minus 4pt%
         \baselineskip 22pt%
         \lineskip     11pt%
         \lineskiplimit 3pt%
        %\parindent    30pt%
         \parindent     0pt%
         \parskip       0pt plus 2pt}%
%
%
% Single space macro for 12 point font.
%
    \gdef\twelvepointsgl{%
         \twelvepoint%
         \abovedisplayskip 14pt plus 4pt minus 4pt%
         \belowdisplayskip 14pt plus 4pt minus 4pt%
         \abovedisplayshortskip 0pt plus 4pt%
         \belowdisplayshortskip 8pt plus 4pt minus 4pt%
         \baselineskip 14pt%
         \lineskip      3pt%
         \lineskiplimit 1pt%
        %\parindent    20pt%
         \parindent     0pt%
         \parskip       0pt plus 1pt}%
%
   \let\doublespace=\twelvepointdbl%
   \let\singlespace=\twelvepointsgl%
%
%   This is a set of macros for switching to 12 point
%
\catcode`@=11\relax%
\def\definetwelve{%
   \font\twelvetext=cmr12 scaled 1000%
   \font\twelvescript=cmr9 scaled 1000%
   \font\twelvescriptscript=cmr7 scaled 1000%
   \font\twelvemathtext=cmmi12 scaled 1000%
   \font\twelvemathscript=cmmi9 scaled 1000%
   \font\twelvemathscriptscript=cmmi7 scaled 1000%
   \font\twelvesymboltext=cmsy10 scaled 1200%             was 1440
   \font\twelvesymbolscript=cmsy9 scaled 1000%
   \font\twelvesymbolscriptscript=cmsy7 scaled 1000%
   \font\twelvemathex=cmex10 scaled 1200%                 was 1440
   \font\twelveboldtext=cmbx12 scaled 1000%
   \font\twelveboldscript=cmbx9 scaled 1000%
   \font\twelveboldscriptscript=cmbx7 scaled 1000%
   \font\twelveslant=cmsl12 scaled 1000%
   \font\twelveitalic=cmti12 scaled 1000%
   \font\twelvetypewriter=cmtt12 scaled 1000%
% Set skew and hyphenation characters
   \skewchar\twelvemathtext='177%
   \skewchar\twelvemathscript='177%
   \skewchar\twelvemathscriptscript='177%
   \skewchar\twelvesymboltext='60%
   \skewchar\twelvesymbolscript='60%
   \skewchar\twelvesymbolscriptscript='60%
   \hyphenchar\twelvetypewriter=-1%
   \global\let\definetwelve=\relax}%
\def\twelvepoint{%
   \definetwelve%
   \textfont0=\twelvetext \scriptfont0=\twelvescript%
      \scriptscriptfont0=\twelvescriptscript%
   \textfont1=\twelvemathtext \scriptfont1=\twelvemathscript%
      \scriptscriptfont1=\twelvemathscriptscript%
   \textfont2=\twelvesymboltext \scriptfont2=\twelvesymbolscript%
      \scriptscriptfont2=\twelvesymbolscriptscript%
   \textfont3=\twelvemathex \scriptfont3=\twelvemathex%
      \scriptscriptfont3=\twelvemathex%
   \textfont\bffam=\twelveboldtext \scriptfont\bffam=\twelveboldscript%
      \scriptscriptfont\bffam=\twelveboldscriptscript%
   \textfont\itfam=\twelveitalic%
   \textfont\slfam=\twelveslant%
   \textfont\ttfam=\twelvetypewriter%
   \def\rm{\fam0\twelvetext}%
   \def\bf{\fam\bffam\twelveboldtext}%
   \def\it{\fam\itfam\twelveitalic}%
   \def\sl{\fam\slfam\twelveslant}%
   \def\tt{\fam\ttfam\twelvetypewriter}%
%
%   Set up \mit, \cal, \oldstyle 
%
   \def\mit{\fam1 }%
   \def\cal{\fam2 }%
   \def\oldstyle{\fam1 \twelvemathtextfont}%
%
%   Set up big etc.
%
\begingroup
\gdef\big##1{{\hbox{$ \left##1\vbox to13.8pt{}\right.\n@space$}}}%   10.2pt
\gdef\Big##1{{\hbox{$ \left##1\vbox to17.4pt{}\right.\n@space$}}}%   13.8pt
\gdef\bigg##1{{\hbox{$\left##1\vbox to21.0pt{}\right.\n@space$}}}%   17.4pt
\gdef\Bigg##1{{\hbox{$\left##1\vbox to24.6pt{}\right.\n@space$}}}%   21.0pt
\endgroup
%
%   Now define a strut box for twelve point.  Should be the height and depth
%   of a \Sigma in math mode.
%
   \setbox\strutbox=\hbox{\vrule height11.5pt depth3.5pt width0pt}%
%
%   Define baselineskip
%
   \normalbaselineskip=14pt%
   \normalbaselines\rm%
}
\catcode`@=12
\twelvepointdbl
%
%
% Double space macro for 17 point font.
%
     \gdef\seventeenpointdbl{%
          \seventeenpoint%
          \abovedisplayskip 22pt plus 6pt minus 6pt%
          \belowdisplayskip 22pt plus 6pt minus 6pt%
          \abovedisplayshortskip  0pt plus 6pt%
          \belowdisplayshortskip 13pt plus 6pt minus 6pt%
          \baselineskip 27pt%
          \lineskip     11pt%
          \lineskiplimit 0pt%
         %\parindent    30pt%
          \parindent     0pt%
          \parskip       0pt plus 6pt}%
%
% Single space macro for 17 point font.
%
    \gdef\seventeenpointsgl{%
         \seventeenpoint%
         \abovedisplayskip 22pt plus 4pt minus 6pt%
         \belowdisplayskip 22pt plus 4pt minus 6pt%
         \abovedisplayshortskip 0pt plus 4pt%
         \belowdisplayshortskip 10pt plus 4pt minus 5pt%
         \baselineskip 19pt%
         \lineskip      2pt%
         \lineskiplimit 0pt%
        %\parindent    20pt%
         \parindent     0pt%
         \parskip       0pt plus 2pt}%
%
    \let\doublespace=\seventeenpointdbl%
    \let\singlespace=\seventeenpointsgl%
%
%   This is a set of macros for switching to 17 point
%
\catcode`@=11\relax%
\newfam\bfslfam%
\def\defineseventeen{%
   \font\seventeentext=cmr17 scaled 1000%
   \font\seventeenscript=cmr12 scaled 1000%
   \font\seventeenscriptscript=cmr9 scaled 1000%
   \font\seventeenmathtext=cmmi12 scaled 1440%
   \font\seventeenmathscript=cmmi12 scaled 1000%
   \font\seventeenmathscriptscript=cmmi9 scaled 1000%
   \font\seventeensymboltext=cmsy10 scaled 1728%
   \font\seventeensymbolscript=cmsy10 scaled 1440%
   \font\seventeensymbolscriptscript=cmsy9 scaled 1000%
   \font\seventeenmathex=cmex10 scaled 1728%
   \font\seventeenboldtext=cmbx12 scaled 1440%
   \font\seventeenboldscript=cmbx12 scaled 1000%
   \font\seventeenboldscriptscript=cmbx9 scaled 1000%
   \font\seventeenslant=cmsl12 scaled 1440%
%  \font\seventeenboldslant=cmbxsl10 scaled 1728%   what about script etc?
   \font\seventeenboldslant=cmbxsl10 scaled 1440%   the best I can do...
   \font\seventeenitalic=cmti12 scaled 1440%
   \font\seventeentypewriter=cmtt12 scaled 1440%
% Set skew and hyphenation characters  -- why not all fonts?
   \skewchar\seventeenmathtext='177%
   \skewchar\seventeenmathscript='177%
   \skewchar\seventeenmathscriptscript='177%
   \skewchar\seventeensymboltext='60%
   \skewchar\seventeensymbolscript='60%
   \skewchar\seventeensymbolscriptscript='60%
   \hyphenchar\seventeentypewriter=-1%
   \global\let\defineseventeen=\relax} % avoids having to re-define fonts
                                       % with evry change to 17 point.
\def\seventeenpoint{%
   \defineseventeen%
   \textfont0=\seventeentext \scriptfont0=\seventeenscript%
      \scriptscriptfont0=\seventeenscriptscript%
   \textfont1=\seventeenmathtext \scriptfont1=\seventeenmathscript%
      \scriptscriptfont1=\seventeenmathscriptscript%
   \textfont2=\seventeensymboltext \scriptfont2=\seventeensymbolscript%
      \scriptscriptfont2=\seventeensymbolscriptscript%
   \textfont3=\seventeenmathex \scriptfont3=\seventeenmathex%
      \scriptscriptfont3=\seventeenmathex%
   \textfont\bffam=\seventeenboldtext \scriptfont\bffam=\seventeenboldscript%
      \scriptscriptfont\bffam=\seventeenboldscriptscript%
   \textfont\itfam=\seventeenitalic%
   \textfont\slfam=\seventeenslant%
   \textfont\ttfam=\seventeentypewriter%
   \def\rm{\fam0\seventeentext}%
   \def\bf{\fam\bffam\seventeenboldtext}%
   \def\it{\fam\itfam\seventeenitalic}%
   \def\sl{\fam\slfam\seventeenslant}%
   \def\tt{\fam\ttfam\seventeentypewriter}%
%
% Creating a new family : bold face slant.
%
% I haven't included any script or scriptscript fonts or the appropriate
% skew and hypenation characters.
%
%  \newfam\bfslfam%  must be defined outside of this macro ie. executed once.
   \textfont\bfslfam=\seventeenboldslant%
   \def\bfsl{\fam\bfslfam\seventeenboldslant}%
   \def\slbf{\fam\bfslfam\seventeenboldslant}%
%
%   Set up \mit, \cal, \oldstyle 
%
   \def\mit{\fam1 }%
   \def\cal{\fam2 }%
   \def\oldstyle{\fam1 \seventeenmathtextfont}%
%
%   Set up big etc.
%
\begingroup
\gdef\big##1{{\hbox{$ \left##1\vbox to17.4pt{}\right.\n@space$}}}%   13.8/10.2pt
\gdef\Big##1{{\hbox{$ \left##1\vbox to21.0pt{}\right.\n@space$}}}%   17.4/13.8pt
\gdef\bigg##1{{\hbox{$\left##1\vbox to24.6pt{}\right.\n@space$}}}%   21.0/17.4pt
\gdef\Bigg##1{{\hbox{$\left##1\vbox to28.2pt{}\right.\n@space$}}}%   24.6/21.0pt
\endgroup
%
%   Now define a strut box for seventeen point.  Should be obtained as the
%   height and depth for \Sigma.
%
   \setbox\strutbox=\hbox{\vrule height21.5pt depth3.5pt width0pt}%
%
%  This definition used by SliTeX.
%
%  \setbox\strutbox=\hbox{\vrule height13.5pt depth5.6pt width0pt}
%
%   Define baselineskip, must agree with definition above.
%
   \normalbaselineskip=19pt%
   \normalbaselines\rm%
}
\catcode`@=12
\seventeenpointdbl
%==============================================================================
\twelvepointsgl
%
\newbox\pgno
\def\pagenumbers{%
\def\folio{\ifnum\pageno>1%
\setbox\pgno=\vbox{\kern+0.5cm\hbox{{\tt-}\number\pageno{\tt-}}}%
\dp\pgno=0pt\ht\pgno=0pt\box\pgno\fi}
\footline={\twelvepoint\hss\folio\hss}%
\headline={\hfil}}
%
\def\nopagenumbers{%
\def\folio{\null}
\headline={\hfil}
\footline={\hfil}}
%
\pagenumbers
%
\vsize=23cm%  for A4 paper (ie. Oz,UK,etc.)
%\vsize=22cm%  for B5 paper (ie. North America)
%
\baselineskip 16pt%       % was 15pt
\lineskip      2pt%       % was 2pt
\lineskiplimit 1pt%
\parindent     0pt%
\parskip       5pt plus 4pt% was 5pt plus 4pt
%
\def\begnarrow{\par\advance\leftskip20pt}
\def\endnarrow{\par\advance\leftskip-20pt}
%
\def\smlskip{\vskip  3pt plus1pt minus1pt}
\def\medskip{\vskip  6pt plus2pt minus2pt}
\def\bigskip{\vskip 12pt plus4pt minus4pt}
%
\def\E(#1){(#1)}
\def\Bar{\overline}
\def\Mymark{$\diamond$}
\def\Ref(#1){\thinspace[#1]\thinspace}
\def\Bf{\seventeenpoint\bf}
%
% --- Define macros for title, address, abstract and sections -----------------
%
\def\TheSecNum{0}%
%
\def\title#1{{\seventeenpoint\bf\halign{\hbox to \hsize{\hfil##\hfil}\cr#1}}}
\def\address#1{\halign{\hbox to \hsize{\hfil##\hfil}\cr#1}}
%
\def\beginabstract{\par\bgroup\tenpoint\vskip1cm%
\centerline{\twelvepoint\bf Abstract}%
\advance\leftskip0cm\advance\rightskip0cm\smlskip}%
%
\def\endabstract{\par\egroup}
%
\newcount\secnum
\newcount\subsecnum
\newcount\subsubsecnum
%
\outer\def\beginsection#1{%
\vskip+4\baselineskip\penalty-500%
\vskip-4\baselineskip%
\vskip 20pt plus 6pt minus 3pt%
\advance\secnum +1\subsecnum=0\subsubsecnum=0\equationnum=0%
{\seventeenpoint\bf\the\secnum.\ #1}%
\def\TheSecNum{\the\secnum}%
\vskip 5pt}%
%
\outer\def\beginsubsection#1{%
\vskip+4\baselineskip\penalty-500%
\vskip-4\baselineskip%
\vskip 10pt plus 3pt minus 2pt%
\advance\subsecnum +1\subsubsecnum=0\equationnum=0%
{\twelvepoint\bf\the\secnum.\the\subsecnum.\ #1}%
\def\TheSecNum{\the\secnum.\the\subsecnum}%
\vskip 5pt}%
%
\outer\def\beginsubsubsection#1{%
\vskip+4\baselineskip\penalty-500%
\vskip-4\baselineskip%
\vskip 10pt plus 3pt minus 2pt%
\advance\subsubsecnum +1%
{\twelvepoint\bf\the\secnum.\the\subsecnum.\the\subsubsecnum.\ #1}%
\def\TheSecNum{\the\secnum.\the\subsecnum}%
\vskip 5pt}%
%
% --- Silently read a file ----------------------------------------------------
%
\newread\tmpfile
%
\def\Input#1{%
\openin\tmpfile=#1
\ifeof\tmpfile\def\readtmp{\message{Can't find #1}}\else
              \def\readtmp{\input #1\relax}\fi
\closein\tmpfile
\readtmp\def\readtmp{\relax}}
%
% --- Define macros for equation numbers --------------------------------------
%
\newread\auxfile
\openin\auxfile=\jobname.aux
\ifeof\auxfile\def\readaux{\relax}\else
              \def\readaux{\input \jobname.aux\relax}\fi
\closein\auxfile
\readaux\def\readaux{\relax}
%
\newwrite\auxfile
\immediate\openout\auxfile=\jobname.aux

\newcount \equationnum \equationnum = 0
\def\numberequation #1{\global\advance\equationnum by 1%
    \expandafter\xdef\csname eqn#1\endcsname{\TheSecNum.\the\equationnum}%
\immediate\write\auxfile{%
    \def\expandafter\noexpand\csname eqn#1\endcsname{%
        \TheSecNum.\the\equationnum}}}

\def\labelequation #1{\expandafter\xdef\csname eqn#1\endcsname{#1}}

\def\eqnlabel#1{\numberequation{#1}}% --- Use this for numbered equations
%\def\eqnlabel#1{\labelequation{#1}}% --- Use this for labeled equations

\def\eqndef#1{\eqnlabel{#1}(\csname eqn#1\endcsname)}
\def\eqnrfr#1{\csname eqn#1\endcsname}
%
% --- Define macros for figure numbers ----------------------------------------
%
\newcount \figurenum \figurenum = 0
\def\numberfigure #1{\global\advance\figurenum by 1%
    \expandafter\xdef\csname fig#1\endcsname{\the\figurenum}%
\immediate\write\auxfile{%
    \def\expandafter\noexpand\csname fig#1\endcsname{%
        \the\figurenum}}}

\def\labelfigure #1{\expandafter\xdef\csname fig#1\endcsname{#1}}

\def\figlabel#1{\numberfigure{#1}}% --- Use this for numbered figures
%\def\figlabel#1{\labelfigure{#1}}% --- Use this for labeled figures

\def\figdef#1{\ignorespaces\figlabel{#1}\csname fig#1\endcsname}
\def\figrfr#1{\csname fig#1\endcsname}
%
% --- Define macros for table numbers -----------------------------------------
%
\newcount \tablenum \tablenum = 0
\def\numbertable #1{\global\advance\tablenum by 1%
    \expandafter\xdef\csname tbl#1\endcsname{\the\tablenum}%
\immediate\write\auxfile{%
    \def\expandafter\noexpand\csname tbl#1\endcsname{%
        \the\tablenum}}}

\def\labeltable #1{\expandafter\xdef\csname tbl#1\endcsname{#1}}

\def\tbllabel#1{\numbertable{#1}}% --- Use this for numbered tables
%\def\tbllabel#1{\labeltable{#1}}% --- Use this for labeled tables

\def\tbldef#1{\tbllabel{#1}\csname tbl#1\endcsname}
\def\tblrfr#1{\csname tbl#1\endcsname}
%
% --- Define macros for section numbers ---------------------------------------
%
\def\numbersection #1{%
    \expandafter\xdef\csname sec#1\endcsname{\TheSecNum}%
\immediate\write\auxfile{%
    \def\expandafter\noexpand\csname sec#1\endcsname{%
        \TheSecNum}}}

\def\labelsection #1{\expandafter\xdef\csname sec#1\endcsname{#1}}

\def\seclabel#1{\numbersection{#1}}% --- Use this for numbered sections
%\def\seclabel#1{\labelsection{#1}}% --- Use this for labeled sections

\def\secdef#1{\seclabel{#1}}%
\def\secrfr#1{{\csname sec#1\endcsname}}%
%
% -----------------------------------------------------------------------------
%
\outer\def\testbreak{%
\vskip0pt plus+2\baselineskip\penalty-250%
\vskip0pt plus-2\baselineskip}
%
\def\RR #1!#2!#3\par{\vskip 0pt plus .1\vsize\penalty -250%
                     \vskip 0pt plus-.1\vsize%
                     \rm\item{\bf [#1]}%              % Ref. number
                     \rm\ignorespaces #2\par\item{}%  % Author
                        \ignorespaces #3\par\par\rm%  % Reference
                     \vskip 5pt}
%
\def\R #1!#2!#3!#4\par{\vskip 0pt plus .1\vsize\penalty -250%
                       \vskip 0pt plus-.1\vsize%
                       \rm\item{\bf [#1]}%              % Ref. number
                       \rm\ignorespaces #2\par\item{}%  % Author
                       \sl\ignorespaces #3\par\item{}%  % Title
                       \rm\ignorespaces #4\par\par\rm%  % Reference
                       \vskip 5pt}

